repro_eval: A Python Interface to Reproducibility Measures of System-oriented IR Experiments

In this work we introduce repro_eval - a tool for reactive reproducibility studies of system-oriented information retrieval (IR) experiments. The corresponding Python package provides IR researchers with measures for different levels of reproduction when evaluating their systems' outputs. By offering an easily extensible interface, we hope to stimulate common practices when conducting a reproducibility study of system-oriented IR experiments.

==> sections/related.tex <==
\section{Related Work}
\label{sec:related}
